WoTify: A platform to bring Web of Things to your devices

The Internet of Things (IoT) has already taken off, together with many Web of Things (WoT) off-the-shelf devices, such as Philips Hue lights and platforms such as Azure IoT. These devices and platforms define their own way of describing the interactions with the devices and do not support the recently published WoT standards by World Wide Web Consortium (W3C). On the other hand, many hardware components that are popular in developer and maker communities lack a programming language independent platform to integrate these components into the WoT, similar to npm and pip for software packages. To solve these problems and nurture the adoption of the W3C WoT, in this paper, we propose a platform to WoTify either existing hardware by downloading new software in them or already existing IoT and WoT devices by describing them with a Thing Description.

==> __latexindent_temp.tex <==
https://www.w3.org/TR/2019/CR-wot-architecture-20190516/
